vqSGD: Vector Quantized Stochastic Gradient Descent

In this work, we present a family of vector quantization schemes \emph{vqSGD} (Vector-Quantized Stochastic Gradient Descent) that provide an asymptotic reduction in the communication cost with convergence guarantees in first-order distributed optimization. In the process we derive the following fundamental information theoretic fact: $\Theta(\frac{d}{R^2})$ bits are necessary and sufficient to describe an unbiased estimator ${\hat{g}}({g})$ for any ${g}$ in the $d$-dimensional unit sphere, under the constraint that $\|{\hat{g}}({g})\|_2\le R$ almost surely. In particular, we consider a randomized scheme based on the convex hull of a point set, that returns an unbiased estimator of a $d$-dimensional gradient vector with almost surely bounded norm. We provide multiple efficient instances of our scheme, that are near optimal, and require only $o(d)$ bits of communication at the expense of tolerable increase in error. The instances of our quantization scheme are obtained using the properties of binary error-correcting codes and provide a smooth tradeoff between the communication and the estimation error of quantization. Furthermore, we show that \emph{vqSGD} also offers strong privacy guarantees.

==> inputs/convergencevqSGD.tex <==
\section{Convergence of vqSGD scheme}

\begin{theorem}
Let ${\cal X} \subset \mathbb{R}^d$ be convex, and let $f: {\cal X} \rightarrow \mathbb{R}$ be unknown, convex, and $L$-smooth. Let $x_0 \in {\cal X}$ be given and let $R^2 := \sup_{x \in {\cal X}} \|x-x_0\|^2$. Let $T > 0$ be fixed. Given repeated, independent access to stochastic gradients with variance bound $\sigma^2$ for $f$, SGD with initial point $x_0$ and constant step sizes $\eta_t = \frac{1}{L + 1/\gamma}$, where $\gamma = \frac{R}{\sigma} \sqrt{\frac{2}{T}}$ achieves
\[
\mathbb{E}\left[ f\left(\frac1T \sum_{t = 0}^T x_t \right)\right] - \min_{x \in {\cal X}} f(x) \le R \sqrt{\frac{2\sigma^2}{T}} + \frac{LR^2}{T}
\]
\end{theorem}

==> inputs/proof-arxiv.tex <==


%Section: Quantization Scheme
\section{Missing Proofs from Section~\ref{sec:quant}}

%Unbiasedness of quantization scheme
\begin{proof}[Proof of Lemma~\ref{lem:unbiased}]
\[\E[Q_C(\p{v})]  = \sum_{i=1}^{|C|} a_i \cdot \p{c_i} = \p{\tilde{v}} = \p{v}.\]
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Variance of general quantization scheme
\begin{proof}[Proof of Lemma~\ref{lem:hull}]
From the definition of the quantization function,
\begin{align*}
\E[ \|\p{v} - Q_C(\p{v}) \|_2^2] &=  \E[\|Q_C(\p{v})\|^2]  - \|\p{v}\|^2 \\
&\le  R^2.
\end{align*}
This is true as $C$ satisfies Condition~\eqref{cond:hull} and therefore, each point $\p{c_i} \in C$ has a bounded norm, $\|\p{c_i}\| \le R$.  
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Variance of SGD
\begin{proof}[Proof of Theorem~\ref{thm:hull}]
Since $\p{\hat{g}}$ is the average of $N$ unbiased estimators, the fact that $\E[\p{\hat{g}}] = \p{g}$ follows from Lemma~\ref{lem:unbiased}.
For the variance computation, note that 
\begin{align*}
\E[\|\p{g} - \p{\hat{g}}\|_2^2] &=\frac{1}{N^2} \left( \sum_{i=1}^N \E[\| \p{g_i} - \p{\hat{g_i}}\|_2^2 ]  \right) \qquad (\mbox{ since } \p{\hat{g_i}} 
\mbox{ is an unbiased estimator of $\p{g}$ })\\
&\le \frac{R^2}{N^2} \sum_{i=1}^N  \| g_i\|^2  \qquad \mbox{(from Lemma~\ref{lem:hull})}.
\end{align*}
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%variance reduction by repetition
\begin{proof}[Proof of Proposition~\ref{prop:var}]
The proof follows simply by linearity of expectations. 
\begin{align*}
\E \left[ \| \p{v} - \p{\hat{v}} \|_2^2 \right] &= \E \left[ \| \frac1s \sum_{i=1}^s \left(\p{v} - Q_C(\p{v}) \right) \|^2 \right] \le \frac{1}{s} \cdot R^2  \qquad  \mbox{(from Lemma~\ref{lem:hull})}. 
\end{align*}
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Section on Constructions 
%\section{Missing Proofs from Section~\ref{sec:constructions} and Other Deterministic Constructions}
%Lower bound



%Characterization


\vspace{0.5in}
%Gaussian

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{0.5in}
%Hadamard / RM_{1, p} construction



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Missing Proofs from Section~\ref{sec:private}}

%SIMPLEX
\begin{proof}[Proof of Proposition~\ref{prop:simplex}]
First we show that the point set $C_{S}$ satisfies Condition~\eqref{cond:hull} with $R=2d$. 
The fact that $\conv(C_S) \subset B_d(\p{0}_d, 2d)$ follows trivially from the observation that each point in $C_S \in B_d(\p{0}_d, 2d)$.

To show that $B_d(\p{0}_d,1) \subset \conv(C_S)$, consider any face of the convex hull, $F_{\p{c}} := \conv(C_S \setminus \{ \p{c} \} )$, for some $\p{c} \in C_S$.  We show that $F_{\p{c}}$ is at an $\ell_2$ distance of at least $1$ from $\p{0}_d$. This in turn shows that any point outside the convex hull must be outside the unit ball as well.  

First consider the case when $\p{c} = -4\p{1}_d$. We observe that the face $F_{\p{c}}$ is contained in the hyperplane $H_{\p{c}}:= \{ \p{x} \in \R^d \mid \frac{1}{\sqrt{d}}{\bf 1}_d^T \p{x} = 2\sqrt{d} \}$, and therefore is at a distance of $O\left(\sqrt{d} \right)$ from the origin. 

Now consider the case when $\p{c} = 2d~\p{e_1}$. Let $\p{w} = \frac{2}{\sqrt{\frac 14 + \frac 1d}}(-\frac 14 + \frac{1}{2d}, \frac{1}{2d}, \ldots, \frac{1}{2d})^T \in \R^d$ be a unit vector. 
 We note that $F_{\p{c}} \subset H_{\p{c}}$, where $H_{\p{c}} := \{ \p{x} \in \R^d \mid \p{w}^T \p{x} = \frac{2}{\sqrt{\frac 14 + \frac 1d}} \}$ is the hyperplane defined by the unit normal vector $\p{w}$ that is at a distance of at least $1$ from $\p{0}_d$. 
 
Since all other faces are symmetric, the proof for the case $\p{c} = 2d~\p{e_i}, i \in [d]$ follows similarly. 

\paragraph{Privacy: } We now show that the quantization scheme is $\eps$-differentially private for any $\eps > \log 7$. From the definition of $\eps$-DP, it is sufficient to show that for any $\p{x}, \p{y} \in B_d(\p{0}_d,1)$ , and any $\p{c} \in C_S$,
\[
 \frac{\Pr[Q_{C_S}(\p{x}) = \p{c}]}{\Pr[Q_{C_S}(\p{y}) = \p{c}]}  \le 7.
\]
Since $\p{x}, \p{y} \in \conv(C_S)$, we can express them as the convex combination of points in $C_S$. Let $\p{x} = \sum_{\p{c} \in C_S} a_c^{(\p{x})}$. Similarly, let $\p{y} = \sum_{\p{c} \in C_S} a_c^{(\p{y})}$. Then, from the construction of the quantization function $Q_{C_S}$, we know that 
\[ 
\frac{\Pr[Q_{C_S}(\p{x}) = \p{c}]}{\Pr[Q_{C_S}(\p{y}) = \p{c}]} = \frac{a_c^{(\p{x}) } }{a_c^{(\p{y})} }. 
\]
We now show that the ratio $\frac{a_c^{(\p{x}) } }{a_c^{(\p{y})} }$ is at most $7$ for any pair $\p{x}, \p{y} \in B_d(\p{0}_d,1)$ and any $\p{c} \in C_S$. The privacy bound follows from this observation. 

First, consider the case  $\p{c} = -4\p{1}_d$. From the closed form solution for any $\p{x} \in \conv(C_S)$ described in Equation~\eqref{eq:simplex_sol}, we know that $a_c^{(\p{x})} = \frac 13 - \frac{\sum_{i=1}^d x_i}{6d}$. For any $\p{x} \in B_d(\p{0}_d,1)$, $\sum_{i=1}^d x_i \in \left[-\|\p{x}\|_1, \|\p{x}\|_1 \right] \subseteq \left[-\sqrt{d}, \sqrt{d} \right]$. Therefore, $a_c^{(\p{x})} \in \left[ \frac13-\frac{1}{6\sqrt{d}},  \frac13+\frac{1}{6\sqrt{d}}  \right]$. It then follows that for any $\p{x}, \p{y} \in B_d(\p{0}_d, 1)$ and $\p{c} = -4\p{1}_d$,
\begin{align*}
 \frac{a_c^{(\p{x}) } }{a_c^{(\p{y})} } &\le \frac{  \frac13+\frac{1}{6\sqrt{d}} }{  \frac13-\frac{1}{6\sqrt{d}}} = 1+\frac{2}{2\sqrt{d} - 1} \le 3
\end{align*}


Now we consider the case when $\p{c} = 2d~\p{e_1}$. Then from the closed from solution in Equation~\eqref{eq:simplex_sol}, we get that for any $\p{x} \in \conv(C_S)$ the coefficient $a_c^{(\p{x})} = \frac{x_1}{2d} \left(1 - \frac{2}{3d} \right) - \frac{\sum_{i=2}^d x_i }{3d^2} + \frac{2}{3d}$. Note that this quantity is maximized for $\p{x} = \p{e_1}$ and minimized for $\p{x} = -\p{e_1}$. Therefore the ratio for any $\p{x}, \p{y} \in B_d(\p{0}_d, 1)$ and $\p{c} = 2d~\p{e_1}$ is at most
\begin{align*}
 \frac{a_c^{(\p{x}) } }{a_c^{(\p{y})} } &\le \frac{  7d-2  }{ d+2 } \le 7
\end{align*}
The ratio for all other vertices can be computed in a similar fashion and is bounded by the same quantity. 
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Hadamard
\begin{proof}[Proof of Proposition~\ref{prop:hadamard}]
First, we show that $C_H$ satisfies Condition~\eqref{cond:hull} with $R=2d$. The fact that $\conv(C_H) \subset B_d(\p{0}_d,2d)$ is trivial and follows since every point in $C_H$ is contained in $B_d(\p{0}_d, 2d)$. 

To show that $B_d(\p{0}_d,1) \subset C_H$, consider any $\p{x} \in B_d(\p{0}_d,1)$, and the closed form solution for the coefficients $a_i$ given by Equation~\eqref{eq:hadamard_sol}. We now show that these coefficients indeed give a convex combination. Note that 
 $a_i := \frac{1}{d+1} \left( 1 +  \frac{\p{c}^T\p{x}}{4d} \right) \ge 0$. This holds since $\p{c}^T\p{x} \ge \|\p{c}\|\|\p{x}\| \ge -2d$.  Moreover, from the property of Hadamard matrices, 
\[
\sum_{i=1}^{d+1} a_i = \frac{1}{d+1}  \begin{bmatrix} 1&\ldots & 1\end{bmatrix} H_p^T \begin{bmatrix} 1\\ \frac{\p{x}}{2\sqrt{d}} \end{bmatrix} = 1.
\]
The last equality follows from the following property of the Hadamard matrices that can be proved using induction. 
\[
\begin{bmatrix} 1&\ldots & 1\end{bmatrix} H_p^T = \begin{bmatrix} 2^p& 0 &\ldots & 0\end{bmatrix}.
\]
Therefore, any $\p{x} \in B_d(\p{0}_d,1)$ can be expressed as a convex combination of the points in $C_H$, \ie, $\p{x} = \sum_{i =1}^{d+1} a_i \p{c_i}$, for $\p{c_i} \in C_H$.


\paragraph{Privacy: } We now show that the quantization scheme is $\eps$-differentially private for any $\eps > \frac{1}{\sqrt{d}}$. From the definition of $\eps$-DP, it is sufficient to show that for any $\p{x}, \p{y} \in B_d(\p{0}_d,1)$, and any $\p{c} \in C_H$,
\[
 \frac{\Pr[Q_{C_H}(\p{x}) = \p{c}]}{\Pr[Q_{C_S}(\p{y}) = \p{c}]}  \le 1+\sqrt{2}
\]
Since $\p{x}, \p{y} \in \conv(C_S)$, we can express them as the convex combination of points in $C_H$. Let $\p{x} = \sum_{\p{c} \in C_H} a_c^{(\p{x})}$. Similarly, let $\p{y} = \sum_{\p{c} \in C_H} a_c^{(\p{y})}$. Then, from the construction of the quantization function $Q_{C_H}$, we know that 
\begin{align}\label{eq:had1}
\frac{\Pr[Q_{C_H}(\p{x}) = \p{c}]}{\Pr[Q_{C_H}(\p{y}) = \p{c}]} = \frac{a_c^{(\p{x}) } }{a_c^{(\p{y})} }. 
\end{align}
From the closed form solution in Equation~\eqref{eq:hadamard_sol}, we know that for any $\p{x} \in \conv(C_H)$, the coefficient of $\p{c}$ in the convex combination of $\p{x}$ is given by $a_c^{(\p{x})} = \frac{1}{d+1} \left( 1 +  \frac{\p{c}^T\p{x}}{4d} \right)$. 
Plugging this in Equation~\eqref{eq:had1}, we get 
\begin{align}\label{eq:had2}
\frac{\Pr[Q_{C_H}(\p{x}) = \p{c}]}{\Pr[Q_{C_H}(\p{y}) = \p{c}]} &= \frac{a_c^{(\p{x}) } }{a_c^{(\p{y})} } 
= \frac{1 +  \frac{\p{c}^T\p{x}}{4d} }{ 1 +  \frac{\p{c}^T\p{y}}{4d}} = 1+ \frac{\frac{\p{c}^T(\p{x}-\p{y})}{4d}}{ 1 +  \frac{\p{c}^T\p{y}}{4d}}  \\
& \leq 1 + \frac{\| \p{c} \|_2\|\p{x} - \p{y} \|_2}{4d - \|\p{c} \|_2}  \qquad \mbox{ for }   \p{y} = -\frac{\p{c}}{\|\p{c}\|_2}\\
& \leq 1+ \frac{2\sqrt{2} d}{4d-2d } \
\intertext{$ (mbox{since } \| \p{x} - \p{y} \|_2 \le \sqrt{2} \mbox{ and } \| \p{c} \|_2 = 2d.)$ }
& =1 + \sqrt{2}
\end{align}
This concludes the proof of Proposition~\ref{prop:hadamard}. 
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Randomised response


==> inputs/unionofpolytopes.tex <==
\section{Union of Polytopes}

The vqSGD scheme can be extended to compute an unbiased estimate of a gradient vector $\p{v} \in B_d(\p{0}_d, 1)$ using a set of polytopes whose union satisfies Condition~\ref{cond:hull}. 

Let $P := \{ P_1, P_2, \ldots, P_t\}$ denote a set $t$ polytopes such that each $P_i := \conv(C_i)$ is a convex hull of a discrete set of points $C_i \subset \mathbb{R}^d$. We note that if $B_d(\p{0}_d, 1) \subset \cup_i P_i \subseteq B_d(\p{0}_d, R)$, then we can design a  quantization scheme $Q_P : B_d(\p{0}_d, 1) \rightarrow \cup_i C_i$ that requires $\log(\sum_i |C_i|)$ bits to communicate an unbiased estimate  $\hat{\p{v}}$ of a gradient vector $\p{v} \in B_d(\p{0}_d, 1)$ with a bound error $\| v - Q_P(\p{v})\|^2 \le R^2$.


Consider an arbitrary (but fixed) ordering of the set of polytopes $P$. For any point $\p{v} \in B_d(\p{0}_d, 1)$, let $P_i$ be the first polytope that contains $\p{v}$. Similar to the vqSGD  scheme, now represent $\p{v}$ as a convex combination of points in $C_i$
\[
\p{v} = \sum_{\p{c} \in C_i}  a_c \p{c} \qquad \sum_{\p{c} \in C_i} a_c = 1, \quad a_c > 0.
\]
The quantization scheme $Q_P$ then returns a vertex $\p{c} \in C_i$ with probability $a_c$. This retains the unbiasedness of the scheme. The error analysis is also similar to that of Lemma~\ref{lem:hull}. 

As noted, vqSGD is a special case of this scheme with $t =1$. However, we remark that this scheme can be used to describe any unbiased quantization scheme. For instance, if we set each $P_i$ to be the unit hypercube that covers the unit sphere in the $i$-th orthant, we get the QSGD \cite{qsgd} scheme. We now formalize this observation. 
\begin{lemma}
\end{lemma}


\subsection{Obtaining vqSGD scheme from union of polytopes}
GIven any set of polytopes $P := \{ P_1, P_2, \ldots, P_t\}$ such that $B_d(\p{0}_d, 1) \subset \cup_i P_i \subseteq B_d(\p{0}_d, R)$, we can obtain a vqSGD quantization scheme by setting $C$ to be the set of points whose convex hull contains the union of polytopes $\cup_i P_i$. Such a point set will then satisfy Condition~\ref{cond:hull} with some $R' > R$, 
\[B_d(\p{0}_d, 1) \subset \conv(C) \subseteq B_d(\p{0}_d, R').\]

Note that if the union of polytopes is in itself a polytope, then the vqSGD scheme obtained reduces the communication cost while incurring the same variance ($R' = R$). 





%extend to union of polytopes. 
%describes any unbiased scheme
%
%description
%relation to vqsgd
%
%qsd, dme as union of polytopes. 
